Pushing the limits of self-supervised ResNets: Can we outperform supervised learning without labels on ImageNet?

Despite recent progress made by self-supervised methods in representation learning with residual networks, they still underperform supervised learning on the ImageNet classification benchmark, limiting their applicability in performance-critical settings. Building on prior theoretical insights from ReLIC [Mitrovic et al., 2021], we include additional inductive biases into self-supervised learning. We propose a new self-supervised representation learning method, ReLICv2, which combines an explicit invariance loss with a contrastive objective over a varied set of appropriately constructed data views to avoid learning spurious correlations and obtain more informative representations. ReLICv2 achieves $77.1\%$ top-$1$ accuracy on ImageNet under linear evaluation on a ResNet50, thus improving the previous state-of-the-art by absolute $+1.5\%$; on larger ResNet models, ReLICv2 achieves up to $80.6\%$ outperforming previous self-supervised approaches with margins up to $+2.3\%$. Most notably, ReLICv2 is the first unsupervised representation learning method to consistently outperform the supervised baseline in a like-for-like comparison over a range of ResNet architectures. Using ReLICv2, we also learn more robust and transferable representations that generalize better out-of-distribution than previous work, both on image classification and semantic segmentation. Finally, we show that despite using ResNet encoders, ReLICv2 is comparable to state-of-the-art self-supervised vision transformers.

==> [arxiv, newest version] ReLICv2/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [arxiv, newest version] ReLICv2/sections/conclusions.tex <==
\section{Discussion}
\label{sec:discussion}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.3cm}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/vit_top1.pdf}
  \caption{Comparison of ImageNet top-1 accuracy between \alpharelic{} and recent vision transformer-based architectures (Swin \citep{liu2021swin} is a fully supervised transformer baseline).
  \label{fig:top1_vit}}
  \vspace{-0.3cm}
\end{wrapfigure}

We proposed a novel self-supervised representation learning method \alpharelic{}, which learns representations by enforcing invariance over views of various sizes and uses saliency masking as part of the data augmentations pipeline to learn representations that are robust to spurious correlations. 
\alpharelic{} sets the new state-of-the-art in self-supervised learning by significantly outperforming previous methods across a wide range of ResNet architectures by up to $+2.3\%$ in linear evaluation on ImageNet. 
Moreover, \alpharelic{} achieves state-of-the art performance on transfer and semi-supervised learning and robustness and out-of-distribution generalization tasks. 
We also show that \alpharelic{} sets a new state-of-the-art when pretrained on JFT-300M and in the process outperforms competing self-supervised methods specifically developed for large and uncurated datasets such as JFT-300M.
On semantic segmentation, our method outperforms competing self-supervised methods, some of them specifically designed for object detection, unlike \alpharelic{}. 
Furthermore, \alpharelic{} is the first method that demonstrates that representations learned without access to labels can consistently outperform a standard supervised baseline on ImageNet which is a first step in making self-supervised learning the go-to approach to learning performant representations.  


%\textcolor{red}{
%We proposed a novel self-supervised representation learning method \alpharelic{} which learns representations by enforcing invariance over multiple different views of varying sizes and saliency masking.
%This enables us to learn robust representations which are more invariant to the above spurious features as evidenced by substantial improvement over existing state-of-the-art in our extensive experimental analysis across a wide range of  downstream settings, tasks and datasets, 
%In particular, \alpharelic{} is the new state-of-the-art in linear evaluation, transfer learning and robustness on ImageNet across ResNet-based self-supervised methods. }


Vision transformers (ViTs) \citep{dosovitskiy2020image} have recently emerged as promising architectures for visual representation learning. 
Figure~\ref{fig:top1_vit} compares recent ViT-based methods against \alpharelic{} using a variety of larger ResNet architectures. 
Notably, \alpharelic{} outperforms recent self-supervised ViT-based methods DINO \citep{caron2021emerging} and MoCov3 \citep{chen2021empirical} as well as exhibits similar performance to EsViT \citep{li2021efficient} for comparable parameter counts despite the fact that these methods use more powerful architectures and more involved training procedures. 
Our results suggest that combining the insights we have developed with \alpharelic{} alongside recent architectural innovations could lead to further improvements in representation learning and more powerful foundation models.  


==> [arxiv, newest version] ReLICv2/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

Large-scale \emph{foundation models} \citep{bommasani2021opportunities}---in particular for language \citep{devlin2018bert, brown2020language} and multimodal domains \citep{radford2021learning}---are an important recent development in representation learning. The idea that massive models can be trained without labels in an unsupervised (or self-supervised) manner and be readily adapted, in a few- or zero-shot setting, to perform well on a variety of downstream tasks is important for many problem areas for which labeled data is expensive or impractical to obtain. 
\emph{Contrastive} objectives have emerged as a successful strategy for representation learning \citep{chen2020simple, he2019momentum, mitrovic2020representation}. However, downstream utility\footnote{Downstream utility is commonly measured by how well a method performs under the standard linear evaluation protocol on ImageNet; see section~\ref{sec:results:linear}.} of these representations has until now never exceeded the performance of supervised training of the same architecture, thus limiting their wide adoption.

\begin{wrapfigure}{R}{0.5\textwidth}
   % \vspace{-0.7cm}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/top1_200.pdf}
  \caption{Top-1 linear evaluation accuracy on ImageNet using ResNet50 encoders with $1\times$, $2\times$ and $4\times$ width multipliers and a ResNet200 encoder with a $2\times$ width multiplier.
  \label{fig:top1}}
  \vspace{-0.5cm}
\end{wrapfigure}

In this work, we tackle the question ``Can we outperform supervised learning without labels on ImageNet?". Thus, our focus is on learning good representations for high-level vision tasks such as image classification.
In supervised learning we have access to label information which provides a signal for what features are relevant for classification.
In unsupervised learning there is no such signal and we have strictly less information available from which to learn compared to the supervised setting.
Thus, the challenge of outperforming supervised learning without labels might seem impossible.
Comparing supervised and contrastive objectives we see that they are two very different approaches to learning representations that yield significantly different representations.
While supervised approaches use labels as targets within a cross-entropy objective, contrastive methods rely on comparing datapoints against other similar and dissimilar datapoints.
Thus, supervised representations end up encoding a small set of highly informative features for downstream performance, while contrastive representations encode many more features with some of these features not related to downstream performance. 
This intuition is also supported by the observation that when visualizing the encoded information of contrastive representations through reconstruction, they are found to retain more detailed information of the original image, such as background and style, than supervised representations \citep{pbordes2021high}. 

Based on this, we hypothesize that one of the key reasons for the current subpar performance of contrastive (and thus self-supervised) representations, is the presence of features which are not directly related to downstream tasks, i.e. so-called \emph{spurious features}.
In general, basing representations on spurious features can have negative consequences for the model's generalization performance and thus avoiding to encode these features is paramount for learning informative representations.

In this paper, we propose to equip self-supervised methods with additional inductive biases to obtain more informative representations and overcome the lack of additional information that supervised methods have access to.
We use as our base self-supervised approach the performant \relic{} method \citep{mitrovic2020representation} which combines a contrastive loss with an invariance loss.
We propose to extend \relic{} by adding inductive biases that penalize the learning of spurious features such as background and style; we denote this method as \alpharelic{}.
First, we propose a new fully unsupervised saliency masking pipeline which enables us to separate the image foreground from its background. We include this novel saliency masking approach as part of the data augmentation pipeline.
Leveraging the invariance loss, this enables us to learn representations that do not rely on the spurious background features.
Second, while \relic{} operates on just two data views of the same size, we extend \alpharelic{} to multiple data views of varying sizes.
Specifically, we argue for learning from a large number of data views of the whole image as well as including a small number of data views that encode only a small part of the image.
The intuition for using smaller crops is that this enables learning of more robust representations as not all features of the foreground might be contained in the small crop. 
Thus, the learned representation is robust against individual object features being absent as it is the case in many real-world settings, e.g. only parts of an object are visible because of occlusion.
On the other hand, using multiple large crops enables us to learn representations that are invariant to object style as the different views correspond to different augmentations.
We extend the contrastive and invariance losses of \relic{} to operate over multiple views of varying sizes.

To showcase the generality and wide applicability of \alpharelic{}, we test it on a wide range of downstream tasks and datasets including image classification, semi-supervised and transfer learning, robustness and out-of-distribution generalisation.
First, we show that \alpharelic{} outperforms by a significant margin previous state-of-the-art self-supervised methods on a wide range of ResNet architectures (ResNet50, ResNet 50 2x, ResNet 50 4x, ResNet101, ResNet152, ResNet200, ResNet 200 2x).  
In terms of top-$1$ classification accuracy on ImageNet, \alpharelic{} achieves $77.1\%$ with ResNet50 which is a $+1.5\%$ improvement over previous work; on larger ResNets, specifically with ResNet200 $2\times$, \alpharelic{} achieves $80.6\%$ top-$1$ accuracy.
Second, we show that \alpharelic{} learns more transferable and robust representations that generalize better out of distribution than previous methods both on image classification as well as semantic segmentation tasks.
Finally, as shown in Figure~\ref{fig:top1}, \alpharelic{} is the first self-supervised representation learning method that outperforms a standard supervised baseline on linear ImageNet evaluation across a wide range of ResNet architectures in a like-for-like comparison.\footnote{Concurrent work in \citep{lee2021compressive} outperforms the same standard supervised baseline only on a ResNet50 $2\times$ encoder.}
Although using ResNets, \alpharelic{} demonstrates comparable performance to recent Vision Transformers \citep{dosovitskiy2020image} (Figure~\ref{fig:top1_vit}). 

These strong experimental results across different vision tasks, learning settings and datasets showcase the generality of our proposed representation learning method. Moreover, we believe that the concepts and results developed in this work could have important implications for wider adoption of self-supervised pre-training in a variety of domains as well as the design of objectives for foundational machine learning systems. 


\noindent\textbf{Summary of contributions.}
We tackle the question “Can we outperform supervised learning without labels on ImageNet?”.
We propose to extend the self-supervised method \relic{} \citep{mitrovic2020representation} with additional inductive biases to learn more informative representations.
We develop a fully unsupervised saliency masking pipeline and use multiple data views of varying sizes to encode these inductive biases. 
The resulting method \alpharelic{} significantly outperforms previous state-of-the-art self-supervised methods across a wide range of ResNet architectures of different depths and width. 
We also highlight the generality of \alpharelic{} representations through state-of-the-art performance on transfer learning, semi-supervised learning, and robustness and out-of-distribution generalization, thus outperforming competing self-supervised methods by a wide margin.
Furthermore, \alpharelic{} is the first self-supervised representation learning method that outperforms a standard supervised model across a wide range of ResNet architecture of different depths and widths.


==> [arxiv, newest version] ReLICv2/sections/method.tex <==
\section{Method} \label{sec:method}

\subsection{Background}

Representation Learning via Invariant Causal Mechanisms (\relic{}) \citep{mitrovic2020representation} learns representations by comparing two differently augmented data views through two mechanisms -- \textit{instance classification}
%, i.e. differentiating individual datapoints from other datapoints, 
and \textit{invariant prediction}.
As is common in prior work, \relic{} tackles the instance classification problem with a contrastive objective, i.e. it learns representations by maximizing the similarity between two differently augmented views of the same datapoint (positives), while minimizing the similarity of that datapoint with other datapoints (negatives).
In addition to that, \relic{} introduces an invariance objective which ensures that the distribution of similarities of a datapoint with its positives and negatives is invariant across augmentations of that datapoint.

Given a randomly sampled batch of datapoints $\{x_{i}\}_{i=1}^{N}$ with $N$ the batch size, \relic{} learns an encoder $f$ that outputs the representation $z$, i.e. $z_{i} = f(x_{i})$. Following \citep{chen2020simple, grill2020bootstrap}, \relic{} creates two views of the data by applying two distinct augmentations randomly sampled from the data augmentation pipeline proposed in \citep{chen2020simple}, i.e. $t, t^{\prime} \sim \mathcal{T}$; this yields two augmented batches $\{x_{i}^{t}\}_{i=1}^{N}$ and $\{x_{i}^{t^{\prime}}\}_{i=1}^{N}$.  
To solve the instance classification problem, \relic{} maximizes the following probability
\begin{equation}
    p(x_i^{t}; x_i^{t^{\prime}})
    = \frac{
     e^{\phi_\tau\left(x_i^{t}, x_i^{t^{\prime}}\right)}
    }{
    e^{\phi_\tau\left( x_i^t, x_i^{t^{\prime}}\right)} + \sum_{x_{j}^{t^\prime} \in \mathcal{N}(x_{i})}  e^{\phi_\tau\left(x_i^{t}, x_j^{t^{\prime}}\right)}
    }
\label{eq:likelihood}
\end{equation}
where $\phi_\tau(x_i, x_j)= \langle h(f(x_i)), q(g(x_j)) \rangle/\tau$ measures the similarity between representations with $\tau$ the temperature parameter.
\relic{} adopts the \emph{target} network setting of \citep{grill2020bootstrap} such that $f$ and $g$ have the same architecture, but the weights of $g$ are an exponential moving average of the weights of $f$; also, $h$ and $q$ are multi-layer perceptrons with $h$ playing the role of the composition of the projector and predictor from \citep{grill2020bootstrap} and $q$ being the exponential moving average of the projector network.; we refer to $f$ and $h$ taken together as the online network, while $g$ and $q$ comprise the target network. 
$\mathcal{N}(x_i)$ represents the set of \emph{negatives}; we uniformly randomly sample a small number of points from the batch to serve as negatives following \citep{mitrovic2020less}.

In order to optimize for invariant prediction, \relic{} introduces an \emph{invariance loss} defined as the Kullback-Leibler divergence between the likelihood of the two augmented data views as 
\begin{equation}
 \KL (p(x_i^{t}) \parallel p(x_i^{t^{\prime}})) = \text{sg}\left[\E_{p(x_i^{t}; x_i^{t^{\prime}})} \log p(x_i^{t}; x_i^{t^{\prime}})\right] 
 -  \E_{p(x_i^{t}; x_i^{t^{\prime}})}\log p(x_i^{t^{\prime}}; x_i^{t})
  \label{eq:invariance}
\end{equation}
and we use the shorthands $p(x_i^{t}) = p(x_i^{t}; x_i^{t^{\prime}})$ and $p(x_i^{t^\prime}) = p(x_i^{t^\prime}; x_i^{t})$.
The invariance loss enforces that the similarity of the representations $ f(x_i^{t})$ and $ f(x_i^{t^\prime})$ \emph{relative} to the positives and negatives is the same; the stop gradient operator, $\text{sg}[\cdot]$, does not affect the computation of the KL-divergence but avoids degenerate solutions during optimization \citep{xie2019unsupervised}.
Taken together, \relic{} learns representations by optimizing the following loss
\begin{equation}
    \mathcal{L} = \sum_{t, t^{\prime}\sim\mathcal{T}} \sum_{i=1}^{N} -\log p(x_i^{t}; x_i^{t^{\prime}}) + \beta\KL (p(x_i^{t}) \parallel p(x_i^{t^{\prime}}))
    \label{eq:loss_relic}
\end{equation}
with $\beta$ a scalar weighting the relative importance of the contrastive and invariance losses.
% losses to the overall objective. 

\subsection{\alpharelic{}} 
We extend Representation Learning via Invariant Causal Mechanisms (\relic{}) \citep{mitrovic2020representation} to include additional inductive biases that prevent the learning of spurious features which are hurting the learning of informative representations.
We encode these inductive biases through a novel fully unsupervised saliency masking pipeline as well as scaling up \relic{} to accommodate multiple data views of varying sizes; we call this method \alpharelic{} and visualize it in Figure \ref{fig:relicv2}.





\noindent\textbf{Saliency masking.} To localize the semantically relevant parts of the image, we propose to use saliency masking. 
In order to separate foreground from background, we develop a fully unsupervised saliency masking pipeline that does not use any additional data.
We learn a saliency masking network without access to any labels or any additional data outside of the ImageNet training set which we also use for pre-training the representation.
We start by using a small subset of ImageNet ($2500$ randomly selected images) and compute initial estimates of saliency masks using a number of handcrafted methods.
Specifically, we use Robust Background Detection  \citep{zhu2014saliency}, Manifold Ranking  \citep{yang2013saliency}, Dense and Sparse Reconstruction  \citep{li2013saliency} and Markov Chain  \citep{jiang2013saliency}. 
% In particular, we sample 2500 random images from ImageNet training set and we compute initial saliency masks for them using the following handcrafted methods:
Next, we use a ResNet50 2x network pretrained on ImageNet in a self-supervised way as the initial saliency detection network.
We adopt the self-supervised refinement mechanism from DeepUSPS\footnote{Note that DeepUSPS cannot be directly applied in our setting as it relies on labelled information and additional datasets (CityScapes) \citep{Cordts2016Cityscapes}.} \citep{deepusps} and incrementally refine the handcrafted saliency masks using a self-supervised objective. Subsequently, the saliency detection network is trained by fusing the refined handcrafted saliency masks.
The trained saliency detection network is used for computing the saliency masks in our pipeline.
During \alpharelic{} pre-training, we randomly apply the saliency masking to input images with a small probability $p_m$. By leveraging images where the background has been removed, \alpharelic{} learns representations that focus on foreground features and are robust to background changes as well as any spurious features that might be found in the background. For more details see  appendix.


\noindent\textbf{Views of varying sizes.}
We propose to enforce invariance over multiple randomly augmented data views of varying sizes to learn more informative representations.
To achieve this, we use a large number of views encoding the whole image as well as a small number of smaller views which contain only a portion of the image.\footnote{Most other methods use only $2$ data views of the whole image.}
As the number of views of the whole image increases so does the variation of object styles seen during training as each view represents a random augmentation manipulating the style of the image. 
Thus, explicitly enforcing invariance over a diverse set of object styles enables us to learn representations which are increasingly invariant to spurious changes in object style.  
Incorporating small views which are random crops of the original image into the learning serves two purposes. 
First, as these views represent a small part of the original image, it is likely that some parts of the objects of interest might be occluded.
Thus, as we learn representations through invariance, using these small views enables us to learn representations which are more robust to object occlusions, a common issue in real-world data.
Note that it is important to use only a small number of small views (in comparison to the number of large views) as using too many small views can result in representations that fail to encode important features as different features might be occluded in different small views and we are learning representations by enforcing invariance.\footnote{For this purpose, we use only $2$ small views in our experiments and provide an ablation analysis on the different number of large and small views.}
Second, we hypothesize that small crops play a synergistic role to saliency masking as taking a small crop of the image is likely to remove potentially large parts of the background; see analysis section for some experimental validation.\footnote{Note that saliency masking is not perfect at removing the background and struggles especially in settings where there is little color contrast between the background and foreground.}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figs/RelicV2.pdf}
  \caption{(a) \alpharelic{} uses saliency masking as part of the data augmentations pipeline and views of various sizes to learn representations that are invariant to spurious correlations. Note that the $L$ (differently augmented) large views are passed through both the online and target networks, while the small $S$ views are only passed through the online network. The learning objective is computed by comparing each of the large and small views passed through the online network with each large view passed through the target network. (b)  The objective used for each comparison combines the contrastive (instance discrimination) loss, i.e the cross-entropy (x-entropy) loss based on the similarity scores, and the invariance loss, i.e. the Kullback-Leibler (KL) divergence between the similarity scores across augmentations. 
\label{fig:relicv2}}
\vspace{-0.5cm}
\end{figure}

\noindent\textbf{Objective.}
\alpharelic{} optimizes a combination of the contrastive and invariance losses across  differently augmented large and small views.
In particular, \alpharelic{} optimizes the following objective:
\begin{align}
    \mathcal{L} = \sum_{i=1}^{N} \sum_{1 \leq l_{1}\leq L}  &
     \biggl( \sum_{1 \leq l_{2} \leq L} \left( 
        -\log p(x_i^{l, t_{l_2}}; x_i^{l, t_{l_{1}}}) +
         \beta\KL (p(x_i^{l, t_{l_{2}}})  \parallel p(x_i^{l, t_{l_{1}}})) \right)+ \\ \nonumber
 & \sum_{1\leq s_{1} \leq S} \left(-\log p(x_i^{s, t_{s_{1}}}; x_i^{l, t_{l_{1}}})  + \beta\KL (p(x_i^{s, t_{s_{1}}}) \parallel p(x_i^{l, t_{l_{1}}}))\right)\biggr)
\end{align}
with $x_{i}^{l, t_{l}}$ a large size view under augmentation $t_{l} \sim \mathcal{T}_{\text{sal}}$, $x_{i}^{s, t_s}$ a small size view under augmentation $t_{s} \sim \mathcal{T}$ and $L$ and $S$ the number of large and small crops, respectively; where $\mathcal{T}_{\text{sal}}$ adds saliency masking with probability $p_m$ on top of $\mathcal{T}$. For more details refer to the appendix. Note that we leverage the differently sized data views in different ways for learning representations. 
We use the large views both for updating the online network as well as for computing learning targets through the target network, i.e. $x_{i}^{l, t_{l_\cdot}}$ appears on both sides of $p$. 
On the other hand, we only use the small views for updating the online network and not as learning targets, i.e. $x_{i}^{s, t_{s_1}}$ appears only on the left hand side of $p$, c.f. Equation \ref{eq:likelihood}. 
% We do not use small views as learning targets as potentially informative parts of the image might be occluded and as such the corresponding features removed from the representation.
% For the selection of the set of negatives, \alpharelic{} follows the approach of \relic{} and uses the simple strategy of uniformly randomly subsampling the batch with $|\mathcal{N}(x_i)|=10$ points.
For the precise architectural and implementation details, as well as a pseudo-code for \alpharelic{} see the appendix.




==> [arxiv, newest version] ReLICv2/sections/outperforming_supervised.tex <==
\section{Evaluating pretrained representations on ImageNet}
\label{sec:results:linear}




We use \alpharelic{} to pretrain representations on the training set of the ImageNet ILSVRC-2012 dataset \citep{russakovsky2015imagenet} without using labels. We evaluate \alpharelic{} representations by training a linear classifier on top of the frozen representation according to the procedure described in \citep{chen2020simple,grill2020bootstrap,dwibedi2021little} and the appendix. From Table~\ref{table.imagenet_linear}, for the ResNet50 encoder, we see that \alpharelic{}  outperforms all previous self-supervised approaches by a significant margin of $+1.5\%$ in terms of top-1 accuracy on the ImageNet test set. \begin{wraptable}{r}{0.4\textwidth}
\vspace{-0.2cm}
\begin{center}
\caption{Top-1 accuracy (in \%) under linear evaluation on the ImageNet test set for a ResNet50 encoder set for different representation learning methods.
}
\label{table.imagenet_linear}
\begin{adjustbox}{max width=0.4\textwidth}
\begin{tabular}{lcc}
\toprule
Method & Top-1 \\
\toprule
\; Supervised \tiny\citep{chen2020simple}   & 76.5 \\ 
\midrule
\; SimCLR {\tiny\citep{chen2020simple}}  & 69.3 \\
\; MoCo v2 \tiny\citep{Chen2020ImprovedBW} & 71.1 \\
\; InfoMin Aug. \tiny\citep{Tian2020WhatMF} & 73.0  \\
\; BYOL \tiny\citep{grill2020bootstrap} & 74.3  \\
\; \relic{} \tiny\citep{mitrovic2020representation} & 74.8 \\ 
\; SwAV \tiny\citep{caron2020unsupervised} & 75.3  \\
\; NNCLR  \tiny\citep{dwibedi2021little}  & 75.6  \\
\; C-BYOL \tiny\citep{lee2021compressive} & 75.6  \\
\; \alpharelic{} (ours) & \textbf{77.1} \\
\hline
\end{tabular}
\end{adjustbox}
\end{center}
\vspace{-0.3cm}
\end{wraptable}
 Moreover, in Table \ref{tab:linear_other_resnets}, note that \alpharelic{} achieves state-of-the-art performance, with margins up to $+2.3\%$ in absolute terms, across a varied set of ResNet encoders of different sizes, spanning ResNet50, ResNet101, ResNet152 and ResNet200 and layer widths of $1\times$, $2\times$ and $4\times$.
ResNet50 with $2\times$ and $4\times$ wider layers has $94$ and $375$ million parameters, respectively.
ResNet101, ResNet152, ResNet200 and ResNet200 $2\times$ have $43$, $58$, $63$ and $250$ million parameters, respectively. Please refer to the appendix for additional results and more details.

Remarkably, from Tables \ref{table.imagenet_linear} and \ref{tab:linear_other_resnets}, we also notice that \alpharelic{} outperforms the standard supervised baselines, across a wide range of ResNet architectures, despite using no label information to pretrain the representation. 
For the ResNet50 encoder, we compare against the supervised baseline model used through the representation learning literature (c.f.~\citep{chen2020simple,grill2020bootstrap,caron2020unsupervised,dwibedi2021little}). 
This model is trained with a cross-entropy loss, a cosine learning rate schedule and full access to labels using the same set of data augmentations as proposed by \citep{chen2020simple}. 
While the recent work of \citep{wightman2021resnet} proposes a series of elaborate optimization and data augmentation tricks to improve the performance of the supervised ResNet50 on ImageNet, we leave the application of these heuristics for future work.
Instead, in this work, we focus on a fair like-for-like comparison between self-supervised methods and supervised learning 
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
 \footnote{Note that using saliency masking to create background augmentations for training the supervised baseline does not improve performance as highlighted in \cite{ryali2021leveraging}}.
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
Refer to the appendix for details about the supervised baselines we used for the other ResNet encoders. 



\begin{table}[h]
\begin{minipage}{.5\linewidth}
    \centering
\begin{tabular}{lc}
\toprule
Method & Top-1  \\
\midrule
\; Supervised \tiny\citep{chen2020simple} &  77.8  \\ 
\; MoCo \tiny\citep{he2019momentum} & 65.4  \\
\; SimCLR \tiny\citep{chen2020simple} & 74.2  \\
\; BYOL \tiny\citep{grill2020bootstrap} &  77.4  \\
\; SwAV \tiny\citep{caron2020unsupervised} &  77.3  \\
\; C-BYOL \tiny\citep{lee2021compressive}  & 78.8  \\
\; \alpharelic{} (ours) &   {\bf 79.0}  \\
\bottomrule
\end{tabular}
\subcaption{ResNet50 $2\times$ encoder.}
\end{minipage}%
    \begin{minipage}{.5\linewidth}
\centering
\begin{tabular}{lc}
\toprule
Method & Top-1  \\
\midrule
\; Supervised \tiny\citep{chen2020simple} &  78.9  \\ 
\; MoCo \tiny\citep{he2019momentum} & 68.6  \\
\; SimCLR \tiny\citep{chen2020simple}  & 76.5 \\
\; SwAV \tiny\citep{caron2020unsupervised} &  77.9  \\
\; BYOL \tiny\citep{grill2020bootstrap} &  78.6  \\
\; \alpharelic{} (ours) &  {\bf 79.4} \\  
\bottomrule
\end{tabular}
\subcaption{ResNet50 $4\times$ encoder.}
\end{minipage}
\begin{minipage}{0.5\linewidth}
\centering
\begin{tabular}{lc}
\toprule
Method & Top-1  \\
\midrule
\; Supervised \tiny\citep{grill2020bootstrap} & 78.0  \\ 
\; BYOL \tiny\citep{grill2020bootstrap} & 76.4  \\
\; \alpharelic{} (ours) & {\bf 78.7}   \\ 
\bottomrule
\end{tabular}
\subcaption{ResNet101 encoder.}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\centering
\begin{tabular}{lc}
\toprule
Method & Top-1  \\
\midrule
\; Supervised \tiny\citep{grill2020bootstrap} & 79.1  \\ 
\; BYOL \tiny\citep{grill2020bootstrap} & 77.3  \\
\; \alpharelic{} (ours) & {\bf 79.3}  \\  
\bottomrule
\end{tabular}
\subcaption{ResNet152 encoder.}
\end{minipage}
\begin{minipage}{0.5\linewidth}
\centering
\begin{tabular}{lc}
\toprule
Method & Top-1  \\
\midrule
\; Supervised \tiny\citep{grill2020bootstrap} & 79.3  \\ 
\; BYOL \tiny\citep{grill2020bootstrap} & 77.8  \\
\; \alpharelic{} (ours) & {\bf 79.8}  \\
\bottomrule
\end{tabular}
\subcaption{ResNet200 encoder.}
\end{minipage}%
\begin{minipage}{0.5\linewidth}
\centering
\begin{tabular}{lc}
\toprule
Method & Top-1 \\
\midrule
\; Supervised \tiny\citep{grill2020bootstrap} &  80.1  \\ 
\; BYOL \tiny\citep{grill2020bootstrap} &  79.6  \\
\; \alpharelic{} (ours) & {\bf 80.6}  \\
\bottomrule
\end{tabular}
\subcaption{ResNet200 $2\times$ encoder.}
\end{minipage}
\caption{Top-1 accuracy (in \%) under linear evaluation on the ImageNet test set for a varied set of ResNet architectures.}
\label{tab:linear_other_resnets}
\end{table}




\newpage

\begin{wrapfigure}{r}{0.6\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/scaling.pdf}
  \caption{ImageNet accuracy obtained by \alpharelic{} as a function of number of images seen during pre-training for several of ResNet architectures (Number of model parameters in brackets).
  \vspace{-0.2cm}
  \label{fig:sup:scaling}}
\end{wrapfigure}


\noindent\textbf{Scaling.} 
Figure~\ref{fig:sup:scaling} shows the ImageNet linear evaluation accuracy obtained by \alpharelic{} representations as a function of the number of images seen during pre-training.
We see that in order to reach $70\%$ accuracy the ResNet50 model requires approximately twice as many iterations as the ResNet295 model, a model we constructed so that it has approximately $3.6\times$ the number of parameters as the ResNet50 (87M vs 24M, respectively). 
This finding is in accordance with other works which show that larger models are more sample efficient (i.e. they require fewer samples to reach a given accuracy) \citep{zhai2021scaling}.



\subsection{Analysis}
\label{sec:analysis}


\noindent\textbf{Class concentration.} To quantify the overall structure of the learned latent space, we examine within- and between-class distances. Figure~\ref{fig:relic_kde} compares the distribution of ratios of between-class and within-class $\ell_2$-distances of the \alpharelic{} representations on the ImageNet test set against those learned by the supervised 
 baseline.\footnote{Both \alpharelic{} and the supervised baseline are trained on the ImageNet training set.} \begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-0.4cm}
    \centering
\includegraphics[width=0.4\textwidth]{figs/kdeplot.pdf}
  \caption{Distribution of the \emph{linear discriminant ratio}: the ratio of between-class distances and within-class distances of embeddings computed on the ImageNet test set. }
\label{fig:relic_kde}
\vspace{-0.3cm}
\end{wrapfigure} 
A higher mean of this distribution means that the representations are better concentrated within the corresponding classes as well as better separated between classes and therefore more easily linearly separable (c.f.~Fisher's linear discriminants \citep{friedman2001elements}). 
We see that \alpharelic's distribution is shifted to the right, i.e. has a higher mean compared to the supervised baseline, suggesting that better representations have been learned. For additional analysis of the  distances between  learned  representations  of closely  related  classes, refer to the appendix. 



\noindent\textbf{Views of varying sizes.} Most prior work uses 2 views of size $224 \times 224$ to learn representations.
RELICv2 proposes instead the use of a large number of views of size $224 \times 224$ combined with a
small number of smaller views of size $96 \times 96$. We ablate the use of different numbers of large and
small views in RELICv2 using only SimCLR augmentations (i.e. without saliency masking). We report below the top-1 ImageNet test performance (under linear evaluation) of a ResNet50 pretrained
for 1000 epoch on ImageNet; $[L, S]$ denotes using L large views and S small views.

\begin{center}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{l|cccccccc}
Views & [2, 0] & [2, 2] & [2, 6] & [4, 0] & [4, 2] & [6, 2] & [8, 2] \\
\hline
Top-1 & 74.8 & 76.2 & 76.0 & 75.5 & {\bf 76.8} & 76.5 & 76.5 \\
\end{tabular}
\end{adjustbox}
\end{center}


There seems to be a performance plateau going beyond 6 large views and a slight performance
penalty going beyond 4 large views. For small views, we also observe performance penalties going
beyond 2 small views, while there is a significant performance boost going from no small views to
2 small views, i.e. $+1.3\%$ in the case of 4 large views. This is almost double the performance improvement one gets from adding 2 large views, i.e the difference between $[2, 0]$ and $[4, 0]$ of $+0.7\%$. This finding supports our hypothesis that small views significantly contribute to learning better representations, but that we only need a small number of them. Note
that our use of large and small views is exactly the opposite as compared to SWaV \citep{caron2018deep} which argue for using smaller views as computationally less expensive alternatives to large
views and rely heavily on using a large number of small views; in particular, they argue for using 2
large views and 6 small views.


\noindent{\textbf{Saliency masking}}. To isolate the contribution of saliency masking, we measure the performance
gain (in terms of top-1 accuracy under linear evaluation on ImageNet) when applying saliency masking to just 2 large views. This improves performance from $74.8\%$ to $75.3\%$, i.e. a gain of $+0.5\%$
which is a boost comparable to having two additional large views (see above). We also explored
using different datasets for pretraining our unsupervised saliency masking pipeline as well as varying the probability with which we apply saliency masking to the inputs and found that RELICv2 is
robust to these choices; see the appendix for details.



\begin{wraptable}{r}{0.5\textwidth}
\vspace{-0.5cm}
\begin{center}
\begin{adjustbox}{max width=0.5\textwidth}
\begin{tabular}{l|l}
 & Top-1 \\
\hline
\; SimCLR {\tiny\citep{chen2020simple}}  & 64.5\% \\
\; SimCLR + [4, 2] + saliency & 66.2\%  (+1.7\%) \\
\hline
\; \relic{} {\tiny\citep{mitrovic2020representation}} & 61.1\%  \\
\; \alpharelic{} (ours) & 67.5\% (+6.4\%) \\
\hline
\end{tabular}
\end{adjustbox}
\end{center}
\vspace{-0.4cm}
\end{wraptable}


\noindent\textbf{Invariance}. To assess the importance of enforcing invariance over background removal and object
styles, we extend SimCLR to use saliency masking, 4 large views and 2 small views, and compare it
to RELICv2. 
We train both methods for 100 epochs
and report top-1 accuracy on ImageNet. 
As we can see from the table, invariance-based methods
profit from multiple views and saliency masking significantly more than purely contrastive methods.
Thus, invariance plays a crucial role in learning better representations.








==> [arxiv, newest version] ReLICv2/sections/review.tex <==
\section{Related work} \label{sec:review}

Recently, \emph{contrastive} approaches have become an important area of research owing to their excellent performance in visual recognition tasks \citep{oord2018representation, bachman2019learning, chen2020simple, he2019momentum, dwibedi2021little, grill2020bootstrap}. 
Moreover, bootstrapping-based learning has also achieved comparable performance \citep{grill2020bootstrap}.
The aforementioned methods implicitly enforce invariance by maximizing the similarity between two views. 
On the other hand, \citep{caron2020unsupervised} incorporates an explicit clustering step as a more direct way of enforcing some notion of invariance.
However, neither of these strategies can be directly linked theoretically to learning more compact representations.  
\citep{mitrovic2020representation} approach invariance from a causal perspective and use an explicit invariance loss in conjunction with a contrastive objective to learn representations.
They show that invariance must be explicitly enforced---via an invariance loss in addition to a contrastive loss---in order to obtain guaranteed generalization performance. 

Background augmentations have recently been proposed as part of the data augmentation pipeline in \citep{zhao2020distilling} and further discussed in concurrent work to our manuscript \citep{ryali2021leveraging}. 
\alpharelic{} differs from these methods in two key points. 
First, we enforce an explicit invariance loss between views with and without background, while \citep{zhao2020distilling} do not have any invariance loss.
Second, \alpharelic{} learns representations using multiple views of varying sizes, while these methods use only two views. 
As a computationally favourable alternative to large views, \citep{caron2020unsupervised} propose to use a large number of small views in addition to the two large views. 
In a notable difference to \citep{caron2020unsupervised}, \alpharelic{} employs small views to increase the representation robustness and proposes to use only a small number of small views. 
Additionally, \alpharelic{} imposes an invariance loss between pairs of large and small views, and uses a large number of large views.
Outside of contrastive learning, \citep{lee2021compressive} take a conditional entropy bottleneck approach which results in better-than-supervised performance albeit only on the ResNet50 (2x) architecture (see Figure~\ref{fig:top1}).
Please refer to the appendix for a more detailed comparison of related works.





==> [arxiv, newest version] ReLICv2/sections/scaling_experiments.tex <==
\vspace{-0.2cm}
\section{Additional experimental results}
\vspace{-0.2cm}
\label{sec:res}

We showcase the generality and wide applicability of \alpharelic{} on transfer, semi-supervised, robustness and out-of-distribution (OOD) generalization tasks when pretraining on ImageNet as well as when we pretrain on the much larger and more complex Joint Foto Tree (JFT-300M) dataset \citep{ sun2017revisiting}. 
Furthermore, we test the transferability of \alpharelic{} representations to more complex vision tasks such as semantic segmentation.
For a complete set of results and experimental details please refer to the appendix.

\subsection{Robustness and OOD generalization}
\label{sec:res:robust}

We evaluate the robustness and out-of-distribution (OOD) generalization of \alpharelic{} on a wide variety of datasets.
We use ImageNetV2 \citep{recht2019imagenet} and ImageNet-C \citep{hendrycks2019benchmarking} to evaluate robustness, while ImageNet-R \citep{hendrycks2021many}, ImageNet-Sketch \citep{wang2019learning} and ObjectNet \citep{barbu2019objectnet} are used to evaluate OOD generalization. 
We evaluate \alpharelic{} representations pretrained on ImageNet on ResNet50 under linear protocol akin to Section \ref{sec:results:linear}, i.e.\ we train a linear classifier on top of the frozen representation using the labelled ImageNet training set; the test evaluation is performed zero-shot, i.e no training is done on the above datasets. 
From Table \ref{table.imagenet_v2_c}, we see that \alpharelic{}
outperforms competing self-supervised models by a wide margin in terms of robustness on ImageNetV2 and ImageNet-C. 
Furthermore, \alpharelic{} also shows better robustness performance than the supervised baseline.
In terms of OOD generalization, \alpharelic{} also learns representations that outperform competing self-supervised methods while being on par with supervised performance. 
For a detailed explanation of the datasets and a full breakdown of the results please see the appendix.

\begin{table}[h]
 \begin{center}
 \vspace{-0.2cm}
% \begin{adjustbox}{max width=\columnwidth}
\caption{Top-1 Accuracy (in \%) under linear evaluation on ImageNetV2 and ImageNet-C (robustness), and ImageNet-R (IN-R), ImageNet-Sketch (IN-S) and ObjectNet (out-of-distribution). ImageNetv2 has three variants -- matched frequency (MF), Threshold 0.7 (T-0.7) and Top Images (TI). The results for ImageNet-C (IN-C) are averaged across the 15 different corruptions.} \label{table.imagenet_v2_c}
 \vspace{-0.1cm}
 \begin{tabular}{lcccc|ccc}
 \toprule
 & \multicolumn{4}{c}{Robustness} & \multicolumn{3}{c}{OOD Generalization} \\
 \toprule
 Method & MF & T-0.7 & Ti & IN-C  & IN-R & IN-S & ObjectNet   \\
 \toprule
 \; Supervised  & 65.1  & 73.9 & 78.4 & 40.9 & 24.0 & 6.1  & 26.6 \\ 
 \midrule
 \; SimCLR \citep{chen2020simple}  & 53.2 & 61.7 & 68.0 & 31.1 & 18.3 & 3.9 & 14.6 \\
 \; BYOL \citep{grill2020bootstrap} & 62.2 & 71.6  & 77.0 & 42.8   & 23.0 & 8.0  &  23.0  \\
 \; \relic{} \citep{mitrovic2020representation} & 63.1 & 72.3 &  77.7 & 44.5 & 23.8 & 9.1 & 23.8 \\
 \; \alpharelic{} (ours) & \textbf{65.3} & \textbf{74.5} & \textbf{79.4} & \textbf{44.8} & \textbf{23.9} & \textbf{9.9} & \textbf{25.9}  \\ 
 \bottomrule
 \end{tabular}
% \end{adjustbox}
 \end{center}
 
 \vspace{-0.6cm}
\end{table}




\subsection{Transfer to other classification datasets and semantic segmentation}
\label{sec:res:transfer}

\paragraph{Classification.} We perform linear evaluation and fine-tuning on a wide range of classification benchmarks. 
We follow established evaluation protocols from the literature as described in the appendix and report standard metrics for each dataset on held-out test sets. 
Figure~\ref{fig:transfer} compares the transfer performance of BYOL, NNCLR and \alpharelic{} pre-trained representations relative to supervised pre-training. 
\alpharelic{} improves upon both the supervised baseline and competing methods, performing best on 7 out of 11 tasks. \alpharelic{} has an average relative improvement
of over $+5\%$ across all tasks---over double that of closest competing self-supervised method NNCLR. 
For detailed results on linear evaluation and fine-tuning see appendix. 

\begin{figure}[h]
\vspace{-0.1cm}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/transfer.pdf}
  \caption{Transfer performance relative to the supervised baseline (a value of 0 indicates equal performance to supervised).}
\label{fig:transfer}
\vspace{-0.2cm}
\end{figure}



\paragraph{Semantic Segmentation.}

\begin{wraptable}{r}{0.5\textwidth}
\vspace{-0.6cm}
\begin{center}
\caption{Transfer performance on semantic segmentation tasks.}
\vspace{-0.3cm}
\label{table.transfer_other_main}
\begin{adjustbox}{max width=0.5\textwidth} 
\centering
\begin{tabular}{l c c}
\toprule
Method & PASCAL & Cityscapes \\
\midrule
BYOL \citep{grill2020bootstrap}  & 75.7 & 74.6 \\
% DetCon \citep{detcon} & 77.3 & \textbf{77.0} \\
ReLICv2 (ours) & {\bf 77.9} & {\bf 75.2} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-0.3cm}
\end{center}
\end{wraptable}

We evaluate the ability of \alpharelic{} to facilitate successful transfer of the learned representations to the PASCAL \citep{Everingham10} and Cityscapes \citep{Cordts2016Cityscapes} semantic segmentation tasks. 
In accordance with~\citep{he2019momentum}, we initialize a fully convolutional backbone with the \alpharelic{} model pretrained on ImageNet.
We fine-tune that model on the PASCAL \texttt{train\_aug2012} set for 45 epochs and report the mean intersection over union (mIoU) on the \texttt{val2012} set. 

The fine-tuning on Cityscapes is done on the \texttt{train\_fine} set for 160 epochs and evaluated on the \texttt{val\_fine} set. 
From Table \ref{table.transfer_other_main} we see that \alpharelic{} significantly outperforms BYOL on both datasets. 
Interestingly, \alpharelic{} outperforms even DetCon \citep{detcon}, a method specifically trained for detection, on PASCAL where it achieves $77.3$ (mIoU).

\subsection{Pretraining on Joint Foto Tree (JFT-300M)} \label{app.results_jft}

We also test how well \alpharelic{} scales to much larger datasets by pretraining representations using the Joint Foto Tree (JFT-300M) dataset which consists of 300 million images from more than 18k classes \citep{ sun2017revisiting}.
We  evaluate the learned representations on the ImageNet test set under the same linear evaluation protocol as described in Section \ref{sec:results:linear}. 

\begin{wraptable}{r}{0.7\textwidth}
\vspace{-0.3cm}
\caption{Top-1 accuracy (in \%) on ImageNet when learning representations using the JFT-300M dataset.}
\vspace{-0.2cm}
\label{table.jft-top1_new}
\begin{center}
\begin{adjustbox}{max width=0.7\columnwidth}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{Top-1} \\
Method & 1000 epochs  & 3000 epochs & $>$4000 epochs \\
\midrule
\; BYOL \tiny\citep{grill2020bootstrap}  &  67.0 & 67.6 & 67.9 (5000 epochs)\\
\; Divide and Contrast \tiny\citep{tian2021divide} & 67.9 & 69.8  & 70.7 (4500 epochs) \\
\; \alpharelic{} (ours) & \textbf{70.3}  & \textbf{71.1} & \textbf{71.4} (5000 epochs) \\ 
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\vspace{-0.5cm}
\end{wraptable}

We compare RELICv2 against BYOL and Divide and Contrast \citep{tian2021divide}, a method
that was specifically designed to handle large and uncurated datasets and represents the current
state-of-art in self-supervised JFT-300M pretraining. Table \ref{table.jft-top1_new} reports the top-1 accuracy when training the various methods using ResNet50 as the backbone for different number of ImageNet equivalent epochs on JFT-300M.
\alpharelic{} improves over Divide and Contrast \citep{tian2021divide} by more than $+2\%$ when training on JFT for 1000 epochs and achieves better overall performance than competing methods while needing a smaller number of training epochs. 
Please refer to the appendix for experimental details and additional results on JFT-300M such as transfer learning, robustness and out-of-distribution evaluation.











